GX-Plug: a Middleware for Plugging Accelerators to Distributed Graph Processing

Recently, research communities highlight the necessity of formulating a scalability continuum for large-scale graph processing, which gains the scale-out benefits from distributed graph systems, and the scale-up benefits from high-performance accelerators. To this end, we propose a middleware, called the GX-plug, for the ease of integrating the merits of both. As a middleware, the GX-plug is versatile in supporting different runtime environments, computation models, and programming models. More, for improving the middleware performance, we study a series of techniques, including pipeline shuffle, synchronization caching and skipping, and workload balancing, for intra-, inter-, and beyond-iteration optimizations, respectively. Experiments show that our middleware efficiently plugs accelerators to representative distributed graph systems, e.g., GraphX and Powergraph, with up-to 20x acceleration ratio.

==> Acknowledgement.tex <==
\section*{Acknowledgments}

This work is supported by NSFC (No. 61772492, 62072428) and the CAS Pioneer Hundred Talents Program. Xike Xie is the corresponding author. We thank Supercomputing Center of USTC for providing the hardware platform and technical support.  

==> MidwareOverview/MO_APIs.tex <==
\subsection{APIs}

\label{subsec:API}

It is important for the middleware to create a series of easy-to-use interfaces to make hardware integration and upper system accessing easy and coder-friendly.
% As a middleware which is designed to serve multiple distributed graph processing systems and computation devices and to make development of both sides more easy, while keeping developments of both sides are separate, two sets of algorithm and interaction APIs with high integrability becomes the key in middleware design.
In our implementation, we design an iteration-based graph algorithm template and an interface set to connect with upper systems.
With these APIs provided, algorithm engineers can focus on the implementation of high-performance graph algorithms,
regardless of upper distributed system details.
Meanwhile, upper system developers can easily access computation resources through daemons,
as well as managing them to cooperate for the global computation in a few lines of code (LOC).

%Here, we show the lists of both daemon algorithm templates and agent interfaces, via which algorithm developer can design algorithm and connect external computation resources easily, and upper system developers can easily access the whole system without consider details inside the middleware and computation devices.

\subsubsection{Algorithm Template}
\label{subsubsec:template}

The APIs of algorithm template follow a unified iterative model and support C++-based code integration, including OpenMP, MPI, CUDA and so on.
There are $3$ steps with computation of an iteration for general multiworker systems, \textit{Message Passing}, \textit{Combining} and \textit{Aggregating}, in which external computation resources can be utilized for computation optimization. Our APIs contain $3$ interfaces, in correspondence to the above $3$ steps: MSGGen(), MSGMerge() and MSGApply().
% , as shown in Listing~\ref{list:apiAlgo}.
% \begin{lstlisting}[language=C++, caption=List of APIs, label={list:apiAlgo}]
% int MSGGen(v *vSet, e *eSet, int edgeNum, msg *mSet);
% int MSGMerge(msg *old, msg *new, int oldMsgNum, int vertexNum);
% int MSGApply(v *vSet, msg *msgSet, int msgNum);
% \end{lstlisting}
With the help of daemon framework, runtime details such as data transferring between the three APIs, runtime order, interactions with upper layers and extra resource management details are hidden to algorithm engineers
% , thus one only needs to focus on application design itself including computation kernel function integration without consideration about other things, while one can still integrate additional management functions into daemon for further optimization
, thus they only focus on the implementation of three APIs for specific graph algorithms.

More, with the separate maintenance of APIs of MSGGen(), MSGMerge() and MSGApply(), upper system developers can arrange the API calls in different orders, so that the middleware is adaptable to various graph computation models, such BSP, GAS, and asynchronous model, shown in Section~\ref{subsubsec:powergraph}. 
{\color{red} \textbf{(To add some links? which can access to the code)}}
% We provide a code example for algorithm engineers to utilize the template for implementing graph applications, in Part~\ref{appendix:codeexample} of the supplementary material.
% Due to the module encapsulation of the daemon-agent framework, algorithm engineers can incorporate further optimization without touching upper system details.

% {
% \color{red}
% \textbf{(Partial answer of GPU hierarchy utilization: reviewer 3.)}
% }

% {
% \color{red}
% \textbf{(Not only implement one utilization, but to adapt various possible utilization)}
% }

\subsubsection{Operation Interfaces}
\label{subsubsec:interface}

To make upper system calls easier to be adapted to agents,  agent accessing is organized into a set of interface functions. With such interface functions of agents, computation daemons can be integrated and cooperated for the global computation invoked by upper systems.
%Upper systems can thus use computation resources located in daemons, as well as integrating and managing them to cooperate for the global computation.

The design of agent interfaces mainly contains three functions, connect(), disconnect() and shutdown() for daemon communication and runtime control, contains two functions, transfer() and update() for data transferring, and function requestX() for computation lifecycle controlling. Here X is one of the three APIs, MSGGen(), MSGMerge() or MSGApply(). upper system users only need to access corresponding functions by inputting proper parameters to get the full control of daemon runtime. Also, it takes merely a few lines of code to connect to upper systems.



% \begin{lstlisting}[language=C++, caption=List of agent interfaces, label={list:apiInterface}]
% int connect(); //Connect to corresponding daemon
% int transfer(v *vSet, e *eSet); //Copy whole graph data to connected daemon
% int update(v *vSet, int *avSet = nullptr, int avCount = -1); //Update modified vertex data to daemon
% void request(); //Call daemon for one iteration execution
% void requestMSGGen(); //Call daemon for one step execution
% void requestMSGMerge();
% void requestMSGApply();
% void disconnect(); //Disconnected from current daemon
% void shutdown(); //Call daemon for self resource release and termination
% \end{lstlisting}





==> RelatedWorks/RW_SingleNodeCPUWorks.tex <==
%\subsection{Single-node CPU-based Systems}

{\bf {Single-node CPU-based Systems}
.}
The single-node CPU-based systems has long been the major platforms for graph analytics, for its ease of operation abstraction and implementation. Boost Graph Library (BGL) and its extended version\cite{Gregor05theparallel} were forerunners of utilizing single-node and multi-core CPU for graph processing.

Many single-node system works focusing on utilizing various components including shared memory in the system level. Ligra\cite{DBLP:conf/ppopp/ShunB13} builds a shared memory architecture based on CilkPlus, and its extension Polymer\cite{DBLP:conf/ppopp/ZhangCC15} provides non-uniform memory access(NUMA) support. Galois\cite{DBLP:conf/sosp/NguyenLP13} chooses to build their system with different operator abstractions that support priority scheduling and dynamic graph processing on subsets of vertices.

However, the coarse-grained parallel programming models are not appropriate for massively parallel processors like GPU and multi-node system, which means those single-node CPU-based system can neither be scaled out by increasing computation node nor be scaled up by utilizing high performance hardwares, and be inevitable when facing challenges in modern graph processing. 

==> SystemImplementation/SI_SystemVIPC.tex <==
\subsection{System V IPC-based Deployment {\color{red} \textbf{\textbf{(Not Necessary?)}}}}

\label{subsec:systemv}

Following the daemon-agent framework, data appeared in an agent given by upper systems can not be directly accessed by daemons, since they belong to different processes with no common memory space, as shown in Section~\ref{subsec:RuntimeIsolation}.
Also, traditional inter-process communication approaches trigger extra data transfers, and significantly degrade the overall system performance.

To tackle this, we resort to kernel functions aided by UNIX System V. There is no extra memory overhead taken for daemons or agents to handle the data transferring.
Instead, a daemon has a unique System V key, that represents a specific System V share memory space in a local distributed node, while an agent has multiple keys to communicate with all daemons attached to the agent.
Agents and daemons can communicate with corresponding System V message queues, facilitating the sequence control of the system.
Also, 
% since data from upper systems or accelerators is kept in the System V share memory, 
{\color{blue}any data updates between agent and daemons can be immediately perceived by the other side, without extra sensing efforts or intermediate transfers, yielding the minimum data transferring between the two ends.}
%{
%\color{red}
%\textbf{(R4Q2)}
%}
%{
%\color{blue}
%Thus, as shown in Figure~\ref{fig:EXP_MidCost}, costs bought by middleware never change no matter the amount of existing deamon-agent framework, and the scalability of integrated system will be only determined by upper system.
%}
Furthermore, pipeline shuffle as shown in Section~\ref{subsec:pipelineShuffle}), can be implemented by changing the order of internal pointers of System V space. Such changes can also be observed by agents for subsequent memory operations, without any extra communication with daemons.

% Furthermore, System V IPC uses a series of user-specific keys to refer to different system V shared memory space and message queues. An agent can have multiple keys, indicating the connections with different daemons.
% During the runtime, daemons of a distributed node use keys in a pre-configured key set to generate different system V shared memory space and message queues, while the agent of the distributed node holds the whole key set. Then, the communication between daemon and agent is done with system V IPC.
%and access different daemons by passing corresponding keys to system V IPC.
%This mechanism supports daemon-agent based distributed system deployment, and makes our middleware can be applied on more specific system environments.

% Following the example used in Section \ref{subsubsec:MultiworkImp}, in a distributed node, multiple daemons, which represent multiple computation resources, can take part in the same computation task, with the help of the agent located in the same node. The agent and daemons communicate with data and msgs through the same System V space, and different System V keys are used to identify the connection with each other. 
